Why is the winner the best?

International benchmarking competitions have become fundamental for the comparative performance assessment of image analysis methods. However, little attention has been given to investigating what can be learnt from these competitions. Do they really generate scientific progress? What are common and successful participation strategies? What makes a solution superior to a competing method? To address this gap in the literature, we performed a multi-center study with all 80 competitions that were conducted in the scope of IEEE ISBI 2021 and MICCAI 2021. Statistical analyses performed based on comprehensive descriptions of the submitted algorithms linked to their rank as well as the underlying participation strategies revealed common characteristics of winning solutions. These typically include the use of multi-task learning (63%) and/or multi-stage pipelines (61%), and a focus on augmentation (100%), image preprocessing (97%), data curation (79%), and postprocessing (66%). The "typical" lead of a winning team is a computer scientist with a doctoral degree, five years of experience in biomedical image analysis, and four years of experience in deep learning. Two core general development strategies stood out for highly-ranked teams: the reflection of the metrics in the method design and the focus on analyzing and handling failure cases. According to the organizers, 43% of the winning algorithms exceeded the state of the art but only 11% completely solved the respective domain problem. The insights of our study could help researchers (1) improve algorithm development strategies when approaching new problems, and (2) focus on open research questions revealed by this work.

==> full_author_list.tex <==
\section{Full author list and affiliations}
\label{sec:author_list}

\subsection{Authors}
% Please don't touch anything here - this content was generated automatically.
Matthias Eisenmann\textsuperscript{1, 2},
Annika Reinke\textsuperscript{1, 2, 3},
Vivienn Weru\textsuperscript{4},
Minu D. Tizabi\textsuperscript{1, 2},
Fabian Isensee\textsuperscript{5, 2},
Tim J. Adler\textsuperscript{1},
Sharib Ali\textsuperscript{6},
Vincent Andrearczyk\textsuperscript{7, 8},
Marc Aubreville\textsuperscript{9},
Ujjwal Baid\textsuperscript{10, 11, 12},
Spyridon Bakas\textsuperscript{10, 11, 12},
Niranjan Balu\textsuperscript{13},
Sophia Bano\textsuperscript{14},
Jorge Bernal\textsuperscript{15},
Sebastian Bodenstedt\textsuperscript{16},
Alessandro Casella\textsuperscript{17},
Veronika Cheplygina\textsuperscript{18},
Marie Daum\textsuperscript{19},
Marleen de Bruijne\textsuperscript{20, 21},
Adrien Depeursinge\textsuperscript{22, 8},
Reuben Dorent\textsuperscript{23, 24},
Jan Egger\textsuperscript{25},
David G. Ellis\textsuperscript{26},
Sandy Engelhardt\textsuperscript{27},
Melanie Ganz\textsuperscript{28, 21},
Noha Ghatwary\textsuperscript{29},
Gabriel Girard\textsuperscript{30, 31, 32},
Patrick Godau\textsuperscript{1, 2, 3, 33},
Anubha Gupta\textsuperscript{34},
Lasse Hansen\textsuperscript{35},
Kanako Harada\textsuperscript{36},
Mattias Heinrich\textsuperscript{35},
Nicholas Heller\textsuperscript{37},
Alessa Hering\textsuperscript{38, 39},
Arnaud Huaulmé\textsuperscript{40},
Pierre Jannin\textsuperscript{40},
Emre Kavur\textsuperscript{1, 2},
Oldřich Kodym\textsuperscript{41},
Michal Kozubek\textsuperscript{42},
Jianning Li\textsuperscript{25},
Hongwei Li\textsuperscript{43},
Jun Ma\textsuperscript{44},
Carlos Martín-Isla\textsuperscript{45},
Bjoern Menze\textsuperscript{46},
Alison Noble\textsuperscript{47},
Valentin Oreiller\textsuperscript{48, 8},
Nicolas Padoy\textsuperscript{49, 50},
Sarthak Pati\textsuperscript{51, 11, 12, 52},
Kelly Payette\textsuperscript{53, 54},
Tim Rädsch\textsuperscript{1, 2},
Jonathan Rafael-Patiño\textsuperscript{31, 32},
Vivek Singh Bawa\textsuperscript{55},
Stefanie Speidel\textsuperscript{56, 57},
Carole H. Sudre\textsuperscript{58, 59, 60, 61},
Kimberlin van Wijnen\textsuperscript{20},
Martin Wagner\textsuperscript{19},
Donglai Wei\textsuperscript{62},
Amine Yamlahi\textsuperscript{1},
Moi Hoon Yap\textsuperscript{63},
Chun Yuan\textsuperscript{13},
Maximilian Zenk\textsuperscript{5, 64},
Aneeq Zia\textsuperscript{65},
David Zimmerer\textsuperscript{5},
Dogu Baran Aydogan\textsuperscript{66, 67},
Binod Bhattarai\textsuperscript{68},
Louise Bloch\textsuperscript{69, 70, 71},
Raphael Brüngel\textsuperscript{69, 70, 71},
Jihoon Cho\textsuperscript{72},
Chanyeol Choi\textsuperscript{73},
Qi Dou\textsuperscript{},
Ivan Ezhov\textsuperscript{74},
Christoph M. Friedrich\textsuperscript{69, 70},
Clifton Fuller\textsuperscript{75},
Rebati Raman Gaire\textsuperscript{76},
Adrian Galdran\textsuperscript{77, 78},
Álvaro García Faura\textsuperscript{79},
Maria Grammatikopoulou\textsuperscript{80},
SeulGi Hong\textsuperscript{81},
Mostafa Jahanifar\textsuperscript{82},
Ikbeom Jang\textsuperscript{83, 84, 85},
Abdolrahim Kadkhodamohammadi\textsuperscript{80},
Inha Kang\textsuperscript{72},
Florian Kofler\textsuperscript{86, 87, 88, 89},
Satoshi Kondo\textsuperscript{90},
Hugo Kuijf\textsuperscript{91},
Mingxing Li\textsuperscript{92},
Minh Huan Luu\textsuperscript{93},
Tomaž Martinčič\textsuperscript{79},
Pedro Morais\textsuperscript{94},
Mohamed A Naser\textsuperscript{75},
Bruno Oliveira\textsuperscript{94, 95, 96},
David Owen\textsuperscript{80},
Subeen Pang\textsuperscript{97},
Jinah Park\textsuperscript{72},
Sung-Hong Park\textsuperscript{93},
Szymon Płotka\textsuperscript{98, 99, 100},
Elodie Puybareau\textsuperscript{101},
Nasir Rajpoot\textsuperscript{82},
Kanghyun Ryu\textsuperscript{102},
Numan Saeed\textsuperscript{103},
Adam Shephard\textsuperscript{82},
Pengcheng Shi\textsuperscript{104},
Dejan Štepec\textsuperscript{79, 105},
Ronast Subedi\textsuperscript{76},
Guillaume Tochon\textsuperscript{101},
Helena Torres\textsuperscript{94, 95, 96},
Helene Urien\textsuperscript{106},
João L. Vilaça\textsuperscript{94},
Kareem Abdul Wahid\textsuperscript{75},
Haojie Wang\textsuperscript{107},
Jiacheng Wang\textsuperscript{107},
Liansheng Wang\textsuperscript{107},
Xiyue Wang\textsuperscript{108},
Benedikt Wiestler\textsuperscript{109},
Marek Wodzinski\textsuperscript{110, 111},
Fangfang Xia\textsuperscript{112, 113},
Juanying Xie\textsuperscript{},
Zhiwei Xiong\textsuperscript{92},
Sen Yang\textsuperscript{114},
Yanwu Yang\textsuperscript{115},
Zixuan Zhao\textsuperscript{113},
Klaus Maier-Hein\textsuperscript{5},
Paul F. Jäger\textsuperscript{116, 2},
Annette Kopp-Schneider\textsuperscript{4},
Lena Maier-Hein\textsuperscript{1, 2, 3, 64, 33}

\subsection{Affiliations}
% Please don't touch anything here - this content was generated automatically.
\textsuperscript{1}Division of Intelligent Medical Systems, German Cancer Research Center (DKFZ), Germany;
\textsuperscript{2}Helmholtz Imaging, German Cancer Research Center (DKFZ), Germany;
\textsuperscript{3}Faculty of Mathematics and Computer Science, Heidelberg University, Germany;
\textsuperscript{4}Division of Biostatistics, German Cancer Research Center (DKFZ), Germany;
\textsuperscript{5}Division of Medical Image Computing, German Cancer Research Center (DKFZ), Germany;
\textsuperscript{6}School of Computing, Faculty of Engineering and Physical Sciences, University of Leeds, UK;
\textsuperscript{7}Institute of Informatics, School of Management, HES-SO Valais-Wallis University of Applied Sciences and Arts Western Switzerland, Switzerland;
\textsuperscript{8}Department of Nuclear Medicine and Molecular Imaging, Lausanne University Hospital, Switzerland;
\textsuperscript{9}Technische Hochschule Ingolstadt, Germany;
\textsuperscript{10}Center for Artificial Intelligence and Data Science for Integrated Diagnostics (AI\textsuperscript{2}D) and Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, USA;
\textsuperscript{11}Department of Pathology and Laboratory Medicine, Perelman School of Medicine, University of Pennsylvania, USA;
\textsuperscript{12}Department of Radiology, Perelman School of Medicine, University of Pennsylvania, USA;
\textsuperscript{13}Department of Radiology, University of Washington, USA;
\textsuperscript{14}Wellcome/EPSRC Centre for Interventional and Surgical Sciences (WEISS) and Department of Computer Science, University College London, UK;
\textsuperscript{15}Universitat Autònoma de Barcelona \& Computer Vision Center, Spain;
\textsuperscript{16}Translational Surgical Oncology - National Center for Tumor Diseases (NCT), Germany;
\textsuperscript{17}Department of Advanced Robotics, Istituto Italiano di Tecnologia, Italy and Department of Electronics, Information and Bioengineering, Politecnico di Milano, Italy;
\textsuperscript{18}IT University of Copenhagen, Denmark;
\textsuperscript{19}Department of General, Visceral and Transplantation Surgery, Heidelberg University Hospital, Germany;
\textsuperscript{20}Biomedical Imaging Group Rotterdam, Department of Radiology and Nuclear Medicine, Erasmus MC, The Netherlands;
\textsuperscript{21}Department of Computer Science, University of Copenhagen, Denmark;
\textsuperscript{22}Institute of Information Systems, University of Applied Sciences Western Switzerland (HES-SO), Switzerland;
\textsuperscript{23}Harvard Medical School, Brigham and Women’s Hospital, USA;
\textsuperscript{24}School of Biomedical Engineering and Imaging Sciences, King's College London, UK;
\textsuperscript{25}Institute for Artificial Intelligence in Medicine (IKIM), University Hospital Essen (AöR), Germany;
\textsuperscript{26}University of Nebraska Medical Center, USA;
\textsuperscript{27}Department of Internal Medicine III, Heidelberg University Hospital, Germany;
\textsuperscript{28}Neurobiology Research Unit, Copenhagen University Hospital, Rigshospitalet, Denmark;
\textsuperscript{29}Arab Academy of Science and Technology, Egypt;
\textsuperscript{30}CIBM Center for Biomedical Imaging, Switzerland;
\textsuperscript{31}Radiology Department, Centre Hospitalier Universitaire Vaudois (CHUV) and University of Lausanne (UNIL), Switzerland;
\textsuperscript{32}Signal Processing Laboratory (LTS5), École Polytechnique Fédérale de Lausanne (EPFL), Switzerland;
\textsuperscript{33}National Center for Tumor Diseases (NCT), Germany;
\textsuperscript{34}SBILab, Department of ECE, IIIT-Delhi, India;
\textsuperscript{35}University of Lübeck, Germany;
\textsuperscript{36}Mechanical Engineering, School of Engineering, The University of Tokyo, Japan;
\textsuperscript{37}University of Minnesota, Department of Computer Science \& Engineering, USA;
\textsuperscript{38}Diagnostic Image Analysis Group, Radboud University Medical Center, The Netherlands;
\textsuperscript{39}Fraunhofer MEVIS, Germany;
\textsuperscript{40}Univ Rennes, INSERM, LTSI - UMR 1099, France;
\textsuperscript{41}Brno University of Technology, Czech Republic;
\textsuperscript{42}Centre for Biomedical Image Analysis, Masaryk University, Czech Republic;
\textsuperscript{43}Department of Quantitative Biomedicine, University of Zurich, Switzerland;
\textsuperscript{44}Department of Mathematics, Nanjing University of Science and Technology, China;
\textsuperscript{45}Departament de Matemàtiques \& Informàtica, Universitat de Barcelona, Spain;
\textsuperscript{46}Biomedical Image Analysis \& Machine Learning, Department of Quantitative Biomedicine, University of Zurich, Switzerland;
\textsuperscript{47}Department of Engineering Science, University of Oxford, UK;
\textsuperscript{48}Institute of Informatics, University of Applied Sciences Western Switzerland (HES-SO), Switzerland;
\textsuperscript{49}ICube, University of Strasbourg, CNRS, France;
\textsuperscript{50}IHU Strasbourg, France;
\textsuperscript{51}Center For Artificial Intelligence And Data Science For Integrated Diagnostics (AI\textsuperscript{2}D) and Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, USA;
\textsuperscript{52}Department of Informatics, Technical University of Munich, Germany;
\textsuperscript{53}Center for MR Research, University Children’s Hospital Zurich, University of Zurich, Switzerland;
\textsuperscript{54}Neuroscience Center Zurich, University of Zurich, Switzerland;
\textsuperscript{55}Visual Artificial Intelligence Laboratory (VAIL), Oxford Brookes University, UK;
\textsuperscript{56}Division of Translational Surgical Oncology, National Center for Tumor Diseases (NCT/UCC) Dresden, Germany;
\textsuperscript{57}Centre for Tactile Internet with Human-in-the-Loop (CeTI), TU Dresden, Germany;
\textsuperscript{58}MRC Unit for Lifelong Health and Ageing, University College London, UK;
\textsuperscript{59}Centre for Medical Image Computing, University College London, UK;
\textsuperscript{60}School of Biomedical Engineering \& Imaging Sciences, King's College London, UK;
\textsuperscript{61}Dementia Research Centre, University College London, UK;
\textsuperscript{62}Computer Science, Boston College, USA;
\textsuperscript{63}Department of Computing and Mathematics, Manchester Metropolitan University, UK;
\textsuperscript{64}Medical Faculty, Heidelberg University, Germany;
\textsuperscript{65}Intuitive Surgical Inc, USA;
\textsuperscript{66}A.I. Virtanen Institute for Molecular Sciences, University of Eastern Finland, Finland;
\textsuperscript{67}Department of Neuroscience and Biomedical Engineering, Aalto University School of Science, Finland;
\textsuperscript{68}University of Aberdeen, UK;
\textsuperscript{69}Department of Computer Science, University of Applied Sciences and Arts Dortmund, Germany;
\textsuperscript{70}Institute for Medical Informatics, Biometry and Epidemiology (IMIBE), University Hospital Essen, Germany;
\textsuperscript{71}Institute for Artificial Intelligence in Medicine (IKIM), University Hospital Essen, Germany;
\textsuperscript{72}School of Computing, Korea Advanced Institute of Science and Technology (KAIST), Republic of Korea;
\textsuperscript{73}Department of Electrical Engineering and Computer Science, Massachusetts Institute of Technology, USA;
\textsuperscript{74}Department of Computer Science, Technical University of Munich, Germany;
\textsuperscript{75}The University of Texas MD Anderson Cancer Center, USA;
\textsuperscript{76}Nepal Applied Mathematics and Informatics Institute for Research (NAAMII), Nepal;
\textsuperscript{77}Universidad Pompeu Fabra, Spain;
\textsuperscript{78}University of Adelaide, Australia;
\textsuperscript{79}XLAB d.o.o., Slovenia;
\textsuperscript{80}Touch Surgery, Medtronic, UK;
\textsuperscript{81}VisionAI, hutom, Republic of Korea;
\textsuperscript{82}Tissue Image Analytics Centre, Department of Computer Science, University of Warwick, UK;
\textsuperscript{83}Hankuk University of Foreign Studies, Republic of Korea;
\textsuperscript{84}Massachusetts General Hospital, USA;
\textsuperscript{85}Harvard Medical School, USA;
\textsuperscript{86}Helmholtz AI, Helmholtz Zentrum München, Germany;
\textsuperscript{87}Department of Informatics, Technical University Munich, Germany;
\textsuperscript{88}TranslaTUM - Central Institute for Translational Cancer Research, Technical University of Munich, Germany;
\textsuperscript{89}Department of Diagnostic and Interventional Neuroradiology, School of Medicine, Klinikum rechts der Isar, Technical University of Munich, Germany;
\textsuperscript{90}Muroran Institute of Technology, Japan;
\textsuperscript{91}UMC Utrecht, The Netherlands;
\textsuperscript{92}University of Science and Technology of China, China;
\textsuperscript{93}Department of Bio and Brain Engineering, Korea Advanced Institute of Science and Technology (KAIST), Republic of Korea;
\textsuperscript{94}2Ai, School of Technology, IPCA, Portugal;
\textsuperscript{95}Algoritmi Center, School of Engineering, University of Minho, Portugal;
\textsuperscript{96}Life and Health Sciences Research Institute, School of Medicine, University of Minho, Portugal;
\textsuperscript{97}Department of Mechanical Engineering, Massachusetts Institute of Technology, USA;
\textsuperscript{98}Sano Centre for Computational Medicine, Poland;
\textsuperscript{99}Informatics Institute, University of Amsterdam, The Netherlands;
\textsuperscript{100}Department of Biomedical Engineering and Physics, Amsterdam University Medical Center, University of Amsterdam, The Netherlands;
\textsuperscript{101}LRE, EPITA, France;
\textsuperscript{102}Artificial Intelligence and Robotics Institute, Korea Institute of Science and Technology, Republic of Korea;
\textsuperscript{103}Mohamed Bin Zayed University of Artificial Intelligence, UAE;
\textsuperscript{104}Harbin Institute of Technology, China;
\textsuperscript{105}University of Ljubljana, Faculty of Computer and Information Science, Slovenia;
\textsuperscript{106}ISEP, France;
\textsuperscript{107}Department of Computer Science at School of Informatics, Xiamen University, China;
\textsuperscript{108}College of Computer Science, Sichuan University, China;
\textsuperscript{109}Department of Neuroradiology, Technical University of Munich, Germany;
\textsuperscript{110}AGH UST, Department of Measurement and Electronics, Poland;
\textsuperscript{111}University of Applied Sciences and Arts Western Switzerland (HES-SO), Switzerland;
\textsuperscript{112}Data Science and Learning Division, Argonne National Laboratory, USA;
\textsuperscript{113}University of Chicago, USA;
\textsuperscript{114}AI Lab, Tencent, China;
\textsuperscript{115}Harbin Institute of Technology (Shenzhen), China;
\textsuperscript{116}Interactive Machine Learning Group, German Cancer Research Center (DKFZ), Germany
